What Language is This? Ask Your Tokenizer

Language Identification (LID) is an important component of many multilingual natural language processing pipelines, where it facilitates corpus curation, training data analysis, and cross-lingual evaluation of large language models. Despite near-perfect performance on high-resource languages, existing systems remain brittle in low-resource and closely related language settings. We introduce UniLID, a simple and efficient LID method based on the UnigramLM tokenization algorithm. In short, to predict a string's language label, we simply ask: under which language's unigram distribution is this string most likely? Our formulation is data- and compute-efficient, supports incremental addition of new languages without retraining existing models, and can naturally be integrated into existing language model tokenization pipelines. Empirical evaluations against widely used baselines, including fasttext, GlotLID-M, and CLD3, show that UniLID achieves competitive performance on standard benchmarks, reaches 69% accuracy with five labeled samples per language and 89% with 25, and delivers large gains on fine-grained dialect identification.

==> tables/calibrated_heldout.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{lrr}
\toprule
\textbf{Method} & \textbf{Macro F1} & \textbf{Ma-FPR (x1e5)} \\
\midrule
\unilid & \corrrev{0.916} & \corrrev{2.03} \\
calibrated \unilid & \corrrev{0.949} & \corrrev{1.78} \\
\fasttext & 0.933 & 2.72 \\
\bottomrule
\end{tabular}
\quad
\begin{tabular}{lrr}
\toprule
\textbf{Comparator} & \textbf{Mean diff} & \textbf{95\% CI} \\
\midrule
\unilid & \corrrev{$+0.034$} & \corrrev{$[+0.029, +0.038]$} \\
\fasttext & \corrrev{$+0.016$} & $[+0.011, +0.022]$ \\
\bottomrule
\end{tabular}
\caption{Left: macro F1 and macro FPR on the held-out part (27{,}002{,}441
lines), outside every calibration-constant selection except the
$100{,}000$-sample \camrev{requirement} (see the provenance table). Right: paired
bootstrap of calibrated \unilid minus each comparator on the held-out part
(10{,}000 resamples over the 1{,}940 languages, percentile interval). FPR
values are multiplied by $10^5$. \camrev{Macro F1 is not invariant to
subsampling, so the held-out levels sit below the full-pool levels of
\cref{tab:lid_main} for every system; the quantity of interest here is the
paired difference.}}
\label{tab:calibrated_heldout}
\end{table}


==> tables/calibrated_nemo.tex <==
\begin{table}[htbp]
\centering
\small
\adjustbox{max width=\linewidth}{
\begin{tabular}{lrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Full pool}} & \textbf{Held-out} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-4}
\textbf{Configuration} & \textbf{Macro F1} & \corrrev{\textbf{Macro FPR ($\times 10^{5}$)}} & \textbf{Macro F1} \\
\midrule
\unilid-Mistral-Nemo (retrained) & \corrrev{0.912} & \corrrev{1.86} & \corrrev{0.895} \\
\quad + unseen-token constant & \corrrev{0.935} & \corrrev{1.79} & \corrrev{0.923} \\
\quad + re-examination (calibrated) & \corrrev{0.950} & \corrrev{1.62} & \corrrev{0.944} \\
\bottomrule
\end{tabular}}
\caption{\corrrev{The two corrections of \cref{sec:calibration}} applied to an independently retrained
\unilid-Mistral-Nemo variant, on the 45{,}377{,}279-line GlotLID-C pool
(full pool) and the 27{,}002{,}441-line held-out subset. FPR values are
multiplied by $10^5$. \corrrev{The retrained baseline is within $0.002$ macro F1 of
the \unilid-Mistral-Nemo row of \cref{tab:lid_main}.}}
\label{tab:calibrated_nemo}
\end{table}


==> tables/calibrated_views.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{lrrrrrrr}
\toprule
& & \multicolumn{3}{c}{\textbf{Global view}} & \multicolumn{3}{c}{\textbf{Within-stratum view}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
\textbf{Train samples} & \textbf{\# Langs} & \unilid & calib.\ \unilid & \fasttext & \unilid & calib.\ \unilid & \fasttext \\
\midrule
$<$500 & 56 & \corrrev{0.596} & \corrrev{0.781} & 0.750 & \corrrev{0.857} & \corrrev{0.820} & 0.915 \\
500--1k & 40 & \corrrev{0.676} & \corrrev{0.893} & 0.861 & \corrrev{0.973} & \corrrev{0.954} & 0.964 \\
1k--12k & 458 & \corrrev{0.894} & \corrrev{0.944} & 0.941 & 0.990 & \corrrev{0.986} & 0.979 \\
12k--18k & 526 & 0.979 & 0.985 & 0.971 & 0.997 & 0.997 & 0.986 \\
18k--35k & 398 & \corrrev{0.962} & 0.965 & 0.953 & 0.992 & 0.992 & 0.981 \\
35k+ & 462 & \corrrev{0.957} & \corrrev{0.956} & 0.941 & 0.958 & \corrrev{0.957} & 0.942 \\
\bottomrule
\end{tabular}
\caption{Mean per-language F1 by training-resource tier under both metric
views, on the 45{,}377{,}279 scored test lines. Global view: every false
positive counts against the predicted language. Within-stratum view: test
examples are restricted to true labels inside the tier, so false positives
arriving from other tiers are excluded (the view used by
\cref{tab:resource-tier}). The two views rank the methods oppositely in the
smallest tiers: calibrated \unilid removes false positives \camrev{\emph{into}} small
languages, which only the global view counts, and re-examination moves some
of the smallest languages' own low-margin lines away, which only the
within-stratum view penalizes.}
\label{tab:calibrated_views}
\end{table*}


==> tables/calibration_provenance.tex <==
\begin{table}[htbp]
\centering
\small
\adjustbox{max width=\linewidth}{
\begin{tabular}{lll}
\toprule
\textbf{Component} & \textbf{Selection data} & \textbf{In scored pool?} \\
\midrule
unseen-token constant \corrrev{$c=-17$} & \camrev{excluded 250k validation sample} & no \\
high-entropy-group membership & \camrev{same excluded 250k sample} & no \\
thresholds, $q_\lang$ & each language's own training data & no \\
$100{,}000$-sample \camrev{requirement} & false-positive profile, full pool & yes \\
proximity bound $21$ & development part (18.0M lines) & yes \\
\bottomrule
\end{tabular}}
\caption{Selected components of calibrated \unilid and the data each was
selected on. The held-out part is outside every row of this table except the
$100{,}000$-sample \camrev{requirement}, which was fixed from a false-positive profile measured
on the whole \camrev{45.0M-line pool remaining after the two draws were
removed,} before the development/held-out split existed.}
\label{tab:calibration_provenance}
\end{table}


==> tables/cld3_refit.tex <==
% New in the corrected round (2026-09-01), re-oriented to the transfer reading (2026-09-02).
% Sources:
%   transferred rows   outputs/rerelease/cld3_calibrated_transfer_2026-09-01.md, section 4
%   subset-fitted row  outputs/rerelease/cld3_regenerated_2026-09-01.md, sections 4 and 6.1
\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l cc cc cc}
\toprule
& \multicolumn{2}{c}{\textbf{GlotLID-C} \small(83 langs)}
& \multicolumn{2}{c}{\textbf{UDHR} \small(80 langs)}
& \multicolumn{2}{c}{\textbf{FLORES-200} \small(77 langs)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\textbf{System} & F1$\uparrow$ & FPR$\downarrow$ & F1$\uparrow$ & FPR$\downarrow$ & F1$\uparrow$ & FPR$\downarrow$ \\
\midrule
\unilid, transferred                        & .972 & 9.99e-5 & .986 & 1.64e-5 & .991 & 3.50e-5 \\
\unilid calibrated, transferred             & .975 & 1.24e-4 & .985 & 2.11e-5 & .992 & 3.83e-5 \\
\midrule
\unilid, fitted to the subset               & .974 & 1.52e-4 & .995 & 5.73e-5 & .997 & 3.93e-5 \\
\bottomrule
\end{tabular}}
\caption{\unilid on the \cld label subsets, when using a model trained on all GlotLID-C languages rather than only the \cld-subset. The \cld-subset columns of \cref{tab:lid_main} instead compare systems each fitted to the subset's languages. Predictions here are left unrestricted for \unilid, so that an error into any of the 1{,}940 labels counts against
the gold language. 
The calibrated system appears in both forms: transferred
here, and fitted to each subset in \cref{tab:lid_main}. The last row is the
subset-fitted \unilid of \cref{tab:lid_main}, repeated for comparison. }
\label{tab:cld3_refit}
\end{table}


==> tables/commonlid.tex <==
\begin{table}[htbp]
\centering
\small
\adjustbox{max width=\linewidth}{
\begin{tabular}{lrr}
\toprule
\textbf{Method} & \textbf{Accuracy} & \textbf{Tag-level macro F1} \\
\midrule
\unilid & \corrrev{0.848} & \corrrev{0.722} \\
\unilid, unseen-token constant only & \corrrev{0.851} & \corrrev{0.720} \\
calibrated \unilid & \corrrev{0.862} & \corrrev{0.717} \\
\bottomrule
\end{tabular}}
\caption{Out-of-domain evaluation on CommonLID (373{,}230 web-domain lines,
109 bare ISO 639-3 tags). A prediction is correct if its language code equals
the gold tag or is a member of the gold macrolanguage; accuracy is
macrolanguage-aware, and tag-level macro F1 averages over the 109 tags.
\corrrev{Calibrated \unilid} raises accuracy because predictions into languages outside the
109-tag set fall from \corrrev{32{,}525} to \corrrev{25{,}994} \camrev{lines}; tag-level macro F1 decreases
slightly because the re-examination also \corrrev{reassigns} some correct low-margin lines,
and the under-resourced languages \corrrev{the two corrections repair} are largely absent
from this tag set.}
\label{tab:commonlid}
\end{table}


==> tables/dialect_stats.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{lrr}
        \toprule
        \textbf{Dialect} & \textbf{Train Samples} & \textbf{Test Size} \\
        \midrule
        FR-BE & 122,369 & 7,543 \\
        FR-CH & 116,490 & 1,027 \\
        FR-FR & 84,402  & 6,351 \\
        FR-CA & 19,041  & 2,169 \\
        ES-ES & 2,616   & 631   \\
        ES-AR & 1,982   & 358   \\
        PT-PT & 1,331   & 356   \\
        PT-BR & 2,556   & 635   \\
        EN-US & 1,342   & 372   \\
        EN-GB & 1,028   & 227   \\
        SR    & 236     & 86    \\
        HR    & 53      & 16    \\
        BS    & 45      & 16    \\
        ME    & 34      & 4     \\
        \bottomrule
    \end{tabular}
    \caption{Train and test set sizes by dialect on DSL-ML 2024. We provide these details to help explain the results observed in \cref{tab:per_language_f1}.}
    \label{tab:dialect_stats}
\end{table}


==> tables/fasttext_epoch_sweep.tex <==
\begin{table*}[!htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\caption{\fasttext per-dialect F1 on DSL-ML 2024 across different training configurations. Macro is the unweighted mean F1 across all 14 dialects. All three BCMS dialects (HR, BS, ME) remain at 0.000 F1 regardless of training budget. \corrrev{Bold marks the best value in a column.}}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l r r r r r r r r r r r r r r r}
\toprule
\textbf{Setting} & \textbf{FR-BE} & \textbf{FR-FR} & \textbf{FR-CA} & \textbf{FR-CH} & \textbf{ES-ES} & \textbf{ES-AR} & \textbf{PT-BR} & \textbf{PT-PT} & \textbf{EN-US} & \textbf{EN-GB} & \textbf{SR} & \textbf{HR} & \textbf{BS} & \textbf{ME} & \textbf{Macro} \\
\midrule
1 Epoch              & 0.6906 & 0.2325 & 0.0000 & 0.2989 & 0.0000 & 0.0000 & 0.0000 & 0.3936 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.1154 \\
5 Epochs             & 0.6894 & 0.3766 & 0.2786 & 0.3997 & 0.8133 & 0.0240 & 0.3812 & 0.5323 & 0.7410 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.3026 \\
10 Epochs            & 0.6832 & 0.4180 & 0.7779 & 0.4676 & 0.8580 & 0.0000 & 0.4995 & 0.5793 & 0.7657 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.3607 \\
10 Epochs, $MC$=10     & 0.6819 & 0.4163 & 0.8055 & \corrrev{\textbf{0.4956}} & 0.8292 & 0.0000 & 0.0243 & 0.5620 & 0.7725 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.3277 \\
100 Epochs, $MC$=10    & 0.6908 & \textbf{0.4434} & \textbf{0.8139} & 0.4457 & \textbf{0.8674} & 0.5426 & 0.6088 & \textbf{0.6208} & 0.8065 & \textbf{0.5949} & 0.8293 & 0.0000 & 0.0000 & 0.0000 & 0.5189 \\
100 Epochs, $MC$=1000 & \textbf{.697} & .434 & .811 & .444 & .833 & \corrrev{\textbf{.686}} & \corrrev{\textbf{.729}} & .609 & \corrrev{\textbf{.815}} & .561 & \corrrev{\textbf{.833}} & .000 & .000 & .000 & \corrrev{\textbf{.532}} \\
\bottomrule
\end{tabular}}
\label{tab:fasttext_epoch_sweep}
\end{table*}


==> tables/latency_glotlid.tex <==
\begin{table}[!htbp]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\caption{Inference latency on GlotLID-C ($|\Lambda|=1940$), evaluated over 45,627,279 samples.}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l r r}
\toprule
\textbf{Method} & \textbf{Latency (ms/sample)}$\downarrow$ & \textbf{Throughput (samples/s)}$\uparrow$ \\
\midrule
\fasttext    & \textbf{0.166} & \textbf{6019} \\
\cld         & 0.187 & 5356 \\
\unilid      & 0.307 & 3253 \\
\bottomrule
\end{tabular}}
\label{tab:latency_glotlid}
\end{table}


==> tables/latency_wili.tex <==
\begin{table}[!htbp]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\caption{Inference latency on WiLI ($|\Lambda|=235$), evaluated over 117,500 samples.}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l r r}
\toprule
\textbf{Method} & \textbf{Latency (ms/sample)}$\downarrow$ & \textbf{Throughput (samples/s)}$\uparrow$ \\
\midrule
\fasttext    & \textbf{0.113} & \textbf{8889} \\
\unilid      & 0.155 & 6435 \\
\cld         & 0.427 & 2340 \\
\bottomrule
\end{tabular}}
\label{tab:latency_wili}
\end{table}


==> tables/lenbias-delta.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Length (chars)} & \textbf{N} & \textbf{Mean $\Delta$} & \textbf{Median $\Delta$} & \textbf{\% fewer} & \textbf{\% same} & \textbf{\% more} \\
\midrule
All misclassified & \corrrev{9,906} & \corrrev{$-0.05$} & $0.00$ & \corrrev{25.29} & \corrrev{52.12} & \corrrev{22.59} \\
\midrule
$<$30    &   \corrrev{2,814} & \corrrev{$-0.05$} & $0.00$ & \corrrev{19.76} & \corrrev{65.28} &  \corrrev{14.96} \\
30--75   &   \corrrev{4,316} & \corrrev{$-0.01$} & $0.00$ & \corrrev{23.96} & \corrrev{53.59} & \corrrev{22.45} \\
75--150  &   \corrrev{2,206} & \corrrev{$-0.04$} & $0.00$ & \corrrev{31.14} & \corrrev{39.30} & \corrrev{29.56} \\
150--300 &   \corrrev{532} & \corrrev{$-0.23$} & $0.00$ & \corrrev{39.66} & \corrrev{26.50} & \corrrev{33.83} \\
300+     &     \corrrev{38} & \corrrev{$-2.13$} & \corrrev{$0.00$} & \corrrev{44.74} & \corrrev{13.16} & \corrrev{42.11} \\
\bottomrule
\end{tabular}
\caption{%
  Token-count length bias on \unilid misclassifications, by input length.
  For each misclassified sample, $\Delta = n_{\mathrm{pred}} - n_{\mathrm{true}}$ is the
  difference in Viterbi segmentation length (in tokens) between the predicted and the true
  language; negative values mean the predicted language uses fewer tokens. \corrrev{Computed over the
  $9{,}906$ misclassifications in the $250{,}000$-line golden subset, the test half of the
  seed-42 $500{,}000$-line draw and the same subset as \cref{tab:lenbias-norm}; the N column is
  therefore not comparable with a count over the full test set.} The mean
  $\Delta$ is negative in every row and \corrrev{grows in magnitude only for inputs above $150$
  characters}, while the median is zero and \corrrev{$52\%$} of errors leave the token count unchanged: a small but systematic bias toward
  fewer-token languages, driven by a minority of samples. \emph{\% fewer/same/more} give the
  share of misclassifications where the predicted language uses fewer, equal, or more tokens
  than the true language. 
}
\label{tab:lenbias-delta}
\end{table*}


==> tables/lenbias-norm.tex <==
\begin{table}[htbp]
\centering
\small
\adjustbox{max width=\columnwidth}{
\begin{tabular}{lrrrr}
\toprule
\textbf{Length (chars)} & \textbf{N} & \textbf{Original} & \textbf{Raw rescore} & \textbf{Normalized} \\
\midrule
$<$30    &  \corrrev{13,708} & \corrrev{0.795} & \corrrev{0.795} & \corrrev{0.494} \\
30--75   & \corrrev{88,503} & \corrrev{0.951} & \corrrev{0.951} & \corrrev{0.776} \\
75--150  & \corrrev{97,861} & \corrrev{0.977} & \corrrev{0.977} & \corrrev{0.883} \\
150--300 &  \corrrev{43,566} & \corrrev{0.988} & \corrrev{0.988} & \corrrev{0.946} \\
300+     &  \corrrev{6,362} & \corrrev{0.994} & \corrrev{0.994} & \corrrev{0.986} \\
\midrule
Overall  & \corrrev{250,000} & \corrrev{0.960} & \corrrev{0.960} & \corrrev{0.837} \\
\bottomrule
\end{tabular}}
\caption{%
  Effect of length-normalizing the per-language log-likelihood on \unilid accuracy, by input
  length. Scores are normalized by dividing the summed token log-probabilities by the
  segmentation length ($\mathrm{score}/n_{\mathrm{tokens}}^{\alpha}$ with $\alpha=1$).
  \emph{Raw rescore} re-runs the unnormalized scorer ($\alpha=0$) through the same code path
  and reproduces the original predictions exactly ($100\%$ agreement), validating the
  implementation. \corrrev{Evaluated on the $250k$-line test half of a $500k$-line uniform sample.} Full normalization lowers overall accuracy from $0.960$ to \corrrev{$0.837$}, with the
  largest degradation on short inputs ($<$30 chars: \corrrev{$0.795 \to 0.494$}) and almost none on long
  inputs: the opposite of where the token-count bias in \cref{tab:lenbias-delta} is
  largest. 
}
\label{tab:lenbias-norm}
\end{table}


==> tables/length_accuracy.tex <==
\begin{table}[t]
\centering
\small
\caption{Accuracy as a function of input sequence length for \unilid and \fasttext on WiLI. All samples in WiLI are $>$ 100 chars long.}
\label{tab:length_accuracy}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\adjustbox{max width=0.8\linewidth}{
\begin{tabular}{l r c c}
\toprule
\textbf{Length (chars)} & \textbf{Samples} & 
\begin{tabular}[c]{@{}c@{}}\textbf{\unilid}\\ Acc. (\%)$\uparrow$\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}\textbf{\fasttext}\\ Acc. (\%)$\uparrow$\end{tabular}\\
\midrule101--150   & 7,845   & \textbf{\corrrev{93.04}} & 90.73 \\
151--200   & 26,652  & \textbf{\corrrev{94.11}} & 92.56 \\
201--300   & 31,449  & \textbf{\corrrev{95.83}} & 94.58 \\
301--500   & 29,494  & \textbf{\corrrev{96.79}} & 96.03 \\
501--1000  & 18,142  & \textbf{\corrrev{96.60}} & 96.25 \\
1000+      & 3,918   & \textbf{\corrrev{96.61}} & 96.30 \\
\midrule
\textbf{Overall} & 117,500 & \textbf{\corrrev{95.64}} & 94.54 \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/lid_main.tex <==
\begin{table*}[ht]
\centering
\small
\caption{Classification results on benchmark evaluation sets.
\unilid variants and \fasttext are trained using the GlotLID-C corpus.
The left columns show results on the full test sets of each benchmark for models that have full coverage of those benchmark's language label set. The right columns show results on the subsets of the benchmarks that \cld has label coverage for. A dash marks a system without coverage of a column's label set; bold marks the best value in a column. \Cref{tab:cld3_refit} reports what the full 1{,}940-language \unilid (i.e., without subsetting to the benchmark's label set) and its calibrated form score on the same benchmarks.}
\label{tab:lid_main}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}
\adjustbox{max width=0.85\textwidth}{
\begin{tabular}{l cc cc cc | cc cc cc}
& \multicolumn{6}{c}{\normalsize \textbf{Full GlotLID-C label set}} &
 \multicolumn{6}{c}{\normalsize \textbf{\cld label set}}\\
\toprule
\textbf{Method} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{GlotLID-C test}\\ \small(1940 labels)\end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{UDHR}\\ \small(366 labels)\end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{FLORES-200}\\ \small(190 labels)\end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{GlotLID-C test}\\ \small(83 languages)\end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{UDHR}\\ \small(80 languages)\end{tabular}} &
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{FLORES-200}\\ \small(77 languages)\end{tabular}} \\

& F1$\uparrow$ & FPR$\downarrow$
& F1$\uparrow$ & FPR$\downarrow$
& F1$\uparrow$ & FPR$\downarrow$
& F1$\uparrow$ & FPR$\downarrow$
& F1$\uparrow$ & FPR$\downarrow$
& F1$\uparrow$ & FPR$\downarrow$ \\
\midrule

% placeholder1
% & -- & --
% & -- & --
% & -- & --
% & -- & --
% & -- & --
% & -- & -- \\



\cld 
& -- & -- 
& -- & -- 
& -- & -- 
& .906 & 5.48e-4
& .965 & 2.52e-4
& .978 & 2.22e-4 \\

\glotlid
& -- & --
& \textbf{.871} & \textbf{1.37e-4}
& \textbf{.968} & \textbf{1.35e-4}
& -- & --
& .994 & \corrrev{\textbf{2.09e-5}}
& \textbf{.999} & \textbf{6.25e-6} \\

\fasttext
& \camrev{.944} & 2.71e-5
& .855 & 1.87e-4
& .938 & 2.38e-4
& \textbf{.990} & \textbf{7.92e-5}
& \textbf{.998} & 2.98e-5
& .998 & 2.96e-5 \\

\midrule
\unilid
& \corrrev{.933} & \corrrev{2.02e-5}
& \corrrev{.856} & \corrrev{1.52e-4}
& \corrrev{.931} & \corrrev{2.83e-4}
& \corrrev{.974} & \corrrev{1.52e-4}
& \corrrev{.995} & \corrrev{5.73e-5}
& \corrrev{.997} & \corrrev{3.93e-5} \\

\unilid (calibrated, \cref{sec:calibration})
& \corrrev{\textbf{.956}} & \camrev{\textbf{1.77e-5}}
& \corrrev{.842} & \corrrev{2.03e-4}
& \corrrev{.932} & 2.91e-4
& \corrrev{.981} & \corrrev{1.48e-4}
& \corrrev{.993} & \corrrev{7.57e-5}
& \corrrev{.997} & \corrrev{3.29e-5} \\

\unilid-Mistral-Nemo
& .912 & \camrev{1.84e-5}
& .836 & 1.79e-4
& .923 & 3.22e-4
& .972 & 1.53e-4
& .992 & \camrev{1.03e-4}
& .994 & 8.05e-5 \\

\unilid-DeepSeek3.2
& .909 & 2.08e-5
& .836 & 1.78e-4
& .914 & 3.42e-4
& .971 & 1.66e-4
& .990 & 1.33e-4
& .994 & 7.92e-5 \\

\unilid-Qwen3
& .904 & 2.55e-5
& .829 & 1.91e-4
& .904 & 3.80e-4
& .964 & 2.27e-4
& .984 & 2.11e-4
& .989 & 1.46e-4 \\





\bottomrule
\end{tabular}}
\end{table*}


==> tables/noise_robustness.tex <==
\begin{table*}[!htbp]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Performance under stochastic character-level perturbation on WiLI (117,500 samples, 235 languages). Each non-whitespace character is replaced with probability $p$. \unilid maintains a small edge at low noise; \fasttext degrades more gracefully at higher noise rates.}
\adjustbox{max width=\linewidth}{
\begin{tabular}{c ccc ccc}
\toprule
& \multicolumn{3}{c}{UniLID} & \multicolumn{3}{c}{fastText} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Noise $p$ & Acc & F1 & FPR & Acc & F1 & FPR \\
\midrule
0\%  & $\mathbf{0.9564}$ & $\mathbf{0.9601}$ & $\mathbf{1.863\times10^{-4}}$ & $0.9527$ & $0.9533$ & $2.023\times10^{-4}$ \\
5\%  & $\mathbf{0.9520}\pm0.0002$ & $\mathbf{0.9553}\pm0.0002$ & $\mathbf{2.051\times10^{-4}}$ & $0.9474\pm0.0003$ & $0.9479\pm0.0003$ & $2.249\times10^{-4}$ \\
10\% & $\mathbf{0.9439}\pm0.0003$ & $\mathbf{0.9468}\pm0.0003$ & $\mathbf{2.398\times10^{-4}}$ & $0.9401\pm0.0007$ & $0.9406\pm0.0007$ & $2.559\times10^{-4}$ \\
25\% & $0.8562\pm0.0003$ & $0.8586\pm0.0001$ & $6.147\times10^{-4}$ & $\mathbf{0.8925}\pm0.0005$ & $\mathbf{0.8922}\pm0.0005$ & $\mathbf{4.592\times10^{-4}}$ \\
50\% & $0.4749\pm0.0009$ & $0.4750\pm0.0010$ & $2.244\times10^{-3}$ & $\mathbf{0.6256}\pm0.0005$ & $\mathbf{0.6272}\pm0.0004$ & $\mathbf{1.600\times10^{-3}}$ \\
\bottomrule
\end{tabular}}
\label{tab:noise_robustness}
\end{table*}


==> tables/per_language_f1.tex <==
\begin{table*}[t]
\centering
\small
\caption{Per-dialect and macro-averaged F1 scores on the DSL-ML 2024 task for French (FR), Spanish (ES), Portuguese (PT), English (EN), and the Bosnian/Croatian/Montenegrin/Serbian family.}
\label{tab:per_language_f1}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\adjustbox{max width=0.7\textwidth}{
\begin{tabular}{l *{4}{c} | *{2}{c} | *{2}{c} | *{2}{c} | *{4}{c} | c}
\toprule
& \multicolumn{4}{c}{\textbf{French}} & \multicolumn{2}{c}{\textbf{Spanish}} & \multicolumn{2}{c}{\textbf{Portuguese}} & \multicolumn{2}{c}{\textbf{English}} & \multicolumn{4}{c}{\textbf{BCMS}} & \\
\cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-15}
\textbf{Model} & BE & FR & CA & CH & ES & AR & BR & PT & US & GB & SR & HR & BS & ME & \textbf{Macro} \\
\midrule
\unilid & .595 & .288 & .798 & \textbf{.456} & \textbf{.867} & \textbf{.832} & \textbf{.816} & \textbf{.724} & \textbf{.855} & \textbf{.815} & \textbf{.929} & \textbf{.788} & \textbf{.609} & \textbf{.750} & \textbf{.723} \\
\fasttext & \textbf{.697} & \textbf{.434} & \textbf{.811} & .444 & .833 & .686 & .729 & .609 & .815 & .561 & .833 & .000 & .000 & .000 & .532 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/resource-tier.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}lrrcccc@{}}
\toprule
 & & & \multicolumn{2}{c}{UniLID} & \multicolumn{2}{c}{fastText} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7}
Train samples / lang & \# Langs & $N_{\text{test}}$ & F1 & FPR & F1 & FPR \\
\midrule
$<\!500$         &  56 & \num{2513}     & \corrrev{0.857} & \corrrev{\num{6.5e-5}} & 0.915 & \num{1.15e-4} \\
$500$\,--\,$1$k    &  40 & \num{5222}     & \corrrev{0.973} & \corrrev{\num{1.0e-5}} & 0.964 & \num{1.9e-5}  \\
$1$k\,--\,$12$k    & 458 & \num{552346}   & 0.990 & \num{8.0e-6} & 0.979 & \num{8.0e-6}  \\
$12$k\,--\,$18$k   & 526 & \num{1151363}  & 0.997 & \num{2.0e-6} & 0.986 & \num{1.0e-5}  \\
$18$k\,--\,$35$k   & 398 & \num{1125105}  & 0.992 & \num{7.0e-6} & 0.981 & \num{1.6e-5}  \\
$35$k$+$           & 462 & \num{42540730} & 0.958 & \corrrev{\num{5.4e-5}} & 0.942 & \num{9.1e-5}  \\
\bottomrule
\end{tabular}
\caption{Performance on the GlotLID-C test set stratified by per-language training-sample count, in the within-stratum view: test examples are restricted to true labels inside each tier, so false positives arriving from other tiers are excluded. \Cref{tab:calibrated_views} repeats this stratification under both metric views. \# Langs is the number of languages in the bucket; $N_{\text{test}}$ is the total number of test instances \camrev{on the 45{,}377{,}279-line scored pool (\cref{app:protocol})}. UniLID matches or exceeds fastText on every bucket except $<\!500$, where the base-vocabulary script bias documented in \cref{tab:script-breakdown} compounds with limited per-language data.}
\label{tab:resource-tier}
\end{table*}


==> tables/script-breakdown.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lrrrr@{}}
\toprule
Script & \# Langs & UniLID & fastText & $\Delta$ \\
\midrule
Latn  & 1{,}700 & \corrrev{0.944} & 0.946 & \corrrev{$-0.002$} \\
Cyrl  &      70 & \corrrev{0.880} & 0.970 & \corrrev{$-0.090$} \\
Arab  &      38 & \corrrev{0.693} & 0.747 & \corrrev{$-0.054$} \\
Deva  &      32 & 0.811 & 0.932 & $-0.121$ \\
Beng  &       6 & \corrrev{0.879} & 0.985 & \corrrev{$-0.106$} \\
Grek  &       4 & \corrrev{0.675} & 0.925 & \corrrev{$-0.250$} \\
Hebr  &       4 & \corrrev{0.738} & 0.967 & \corrrev{$-0.229$} \\
Armn  &       2 & \corrrev{0.972} & 0.986 & \corrrev{$-0.014$} \\
Other &      82 & 0.937 & 0.973 & $-0.036$ \\
\bottomrule
\end{tabular}
\caption{Macro-F1 on the GlotLID-C test set stratified by Unicode script (ISO 15924), in the within-stratum view: test examples are restricted to true labels inside each script group, so false positives arriving from other scripts are excluded. The two single-language scripts (Korean, Japanese) are excluded from the Other row. $\Delta = \text{F1}(\text{UniLID}) - \text{F1}(\text{fastText})$. UniLID matches fastText on Latin-script languages but underperforms on every non-Latin script, with the largest gaps on Greek, Hebrew, and Devanagari. We attribute this to the training distribution of the base vocabulary $V$, which is dominated by Latin-script text in GlotLID-C.}
\label{tab:script-breakdown}
\end{table}


==> tables/tatoeba_udhr_comparison.tex <==
\begin{table}[t]
\centering
\small
\caption{Macro-averaged F1 and false positive rate (FPR) of \fasttext and \unilid trained on WiLI and evaluated on the Tatoeba and UDHR benchmarks.}
\label{tab:tatoeba_udhr_comparison}
\setlength{\tabcolsep}{7pt}
% \renewcommand{\arraystretch}{1.}
\adjustbox{max width=\linewidth}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Method} &
    \multicolumn{2}{c}{\textbf{Tatoeba} (201 langs)} &
    \multicolumn{2}{c}{\textbf{UDHR} (142 langs)} \\
    & \textbf{Macro F1}$\uparrow$ & \textbf{Macro FPR}$\downarrow$
    & \textbf{Macro F1}$\uparrow$ & \textbf{Macro FPR}$\downarrow$ \\
    \midrule
    \fasttext & 0.160 & 3.58e-3 & 0.849 & 6.07e-4 \\
    \unilid & \textbf{\corrrev{0.420}} & \textbf{\corrrev{9.23e-4}} & \textbf{\corrrev{0.866}} & \textbf{\corrrev{5.86e-4}} \\
    \bottomrule
    \end{tabular}%
}
\end{table}


==> tables/training_time.tex <==
\begin{table}[!htbp]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\caption{Wall-clock training time on the GlotLID-C training set. \unilid splits the training cost across base tokenizer learning (1k samples per language) and per-language EM re-estimation; \fasttext is trained on the full training set for 100 epochs.}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l r}
\toprule
\textbf{Method} & \textbf{Total Time (s)}$\downarrow$ \\
\midrule
\unilid              & \textbf{17{,}776} \\
\fasttext (100 ep.)  & $\sim$163{,}000 \\
\bottomrule
\end{tabular}}
\label{tab:training_time}
\end{table}


==> tables/unilid_llm_comparison.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l c c}
\toprule
\textbf{Method} & \textbf{Macro F1}$\uparrow$ & \textbf{Macro FPR}$\downarrow$ \\
\midrule
\unilid (base)              & \textbf{\corrrev{0.960}} & \textbf{\corrrev{1.863e-4}} \\
\fasttext    & \corrrev{0.953} & 2.331e-4 \\
\hdashline
\unilid-Mistral-Nemo      & \corrrev{0.959} & \corrrev{1.894e-4} \\
\unilid-Mistral      & \corrrev{0.920} & \corrrev{3.380e-4} \\
\unilid-LLaMA3.2     & \corrrev{0.954} & \corrrev{2.081e-4}\\
\unilid-LLaMA2       & \corrrev{0.910}& \corrrev{3.733e-4} \\
\unilid-DeepSeek3.2       & \corrrev{0.955} & \corrrev{2.048e-4} \\
\unilid-Qwen3       & \corrrev{0.948} & \corrrev{2.341e-4} \\
\bottomrule
\end{tabular}}
\caption{Macro-averaged F1 and FPR of different LID systems on WiLI; \camrev{the rows below the dashed line} are variants of \unilid trained using the base tokenizers from open-source LLMs.}
\label{tab:unilid_llm_comparison}
\end{table}


==> tables/viterbi_vs_marginal.tex <==
\begin{table}[!htbp]
\centering
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\caption{Comparison of Viterbi decoding versus exact marginalization (forward algorithm) at inference time on GlotLID-C. \corrrev{Inference under marginalization takes approximately $1.7\times$ the time of Viterbi decoding, and macro F1 is 0.002 higher.}}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l c c}
\toprule
\textbf{Decoding} & \textbf{Accuracy}$\uparrow$ & \textbf{Macro F1}$\uparrow$ \\
\midrule
\unilid (Viterbi)         & 0.961 & \corrrev{0.933} \\
\unilid (Marginalization) & \corrrev{0.961} & \corrrev{\textbf{0.935}} \\
\bottomrule
\end{tabular}}
\label{tab:viterbi_vs_marginal}
\end{table}


==> tables/vocab_size_efficiency.tex <==
\begin{table}[!h]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\caption{Effect of base tokenizer vocabulary size on \unilid performance and inference efficiency evaluated on WiLI. \corrrev{Macro F1 and macro FPR come from base tokenizers retrained for this table; at $100$k the retrained vocabulary contains the same $100{,}000$ tokens as the published one, in a different order at 132 of the positions. The latency and throughput columns are the original measurements and were not re-measured on the retrained models.}}
\adjustbox{max width=\linewidth}{
\begin{tabular}{c c c c c}
\hline
\textbf{Vocab Size} &
\textbf{Macro F1}$\uparrow$ &
\textbf{Macro FPR}$\downarrow$ &
\textbf{Latency (ms)}$\downarrow$ &
\textbf{Samples/s}$\uparrow$ \\
\hline
10k   & \corrrev{0.944} & \corrrev{2.556e-4} & 0.113 & 8891.99 \\
20k   & \corrrev{0.950} & \corrrev{2.303e-4} & 0.119 & 8421.68 \\
50k   & \corrrev{0.957} & \corrrev{2.015e-4} & 0.147 & 6818.08 \\
100k  & \corrrev{0.960} & \corrrev{1.863e-4} & 0.175 & 5717.68 \\
200k  & \textbf{\corrrev{0.9606}} & \textbf{\corrrev{1.8418e-4}} & 0.2328 & 4296.45 \\
\hline
\end{tabular}}
\label{tab:vocab_size_efficiency}
\end{table}

